DeepHGCN: Toward Deeper Hyperbolic Graph Convolutional Networks

Hyperbolic graph convolutional networks (HGCNs) have demonstrated significant potential in extracting information from hierarchical graphs. However, existing HGCNs are limited to shallow architectures due to the computational expense of hyperbolic operations and the issue of over-smoothing as depth increases. Although treatments have been applied to alleviate over-smoothing in GCNs, developing a hyperbolic solution presents distinct challenges since operations must be carefully designed to fit the hyperbolic nature. Addressing these challenges, we propose DeepHGCN, the first deep multi-layer HGCN architecture with dramatically improved computational efficiency and substantially reduced over-smoothing. DeepHGCN features two key innovations: (1) a novel hyperbolic feature transformation layer that enables fast and accurate linear mappings, and (2) techniques such as hyperbolic residual connections and regularization for both weights and features, facilitated by an efficient hyperbolic midpoint method. Extensive experiments demonstrate that DeepHGCN achieves significant improvements in link prediction and node classification tasks compared to both Euclidean and shallow hyperbolic GCN variants.

==> table/exp_lpnc.tex <==
\begin{tabular}{@{}llcclcclcclcc@{}}
\toprule
\textbf{Dataset ($\delta$)} &  & \multicolumn{2}{c}{\textbf{Airport ($\delta = 1$)}}     &  & \multicolumn{2}{c}{\textbf{PubMed ($\delta =   3.5$)}}  &  & \multicolumn{2}{c}{\textbf{CiteSeer ($\delta =   5$)}}  &  & \multicolumn{2}{c}{\textbf{Cora ($\delta = 11$)}}       \\ \cmidrule(lr){3-4} \cmidrule(lr){6-7} \cmidrule(lr){9-10} \cmidrule(l){12-13} 
\textbf{Task}               &  & LP                         & NC                         &  & LP                         & NC                         &  & LP                         & NC                         &  & LP                         & NC                         \\ \midrule
MLP                         &  & 89.81${\pm 0.56}$          & 68.90${\pm 0.46}$          &  & 83.33${\pm 0.56}$          & 72.40${\pm 0.21}$          &  & 93.73${\pm 0.63}$          & 59.53${\pm 0.90}$          &  & 83.33${\pm 0.56}$          & 51.59${\pm 1.28}$          \\
HNN                         &  & 90.81${\pm 0.23}$          & 80.59${\pm 0.46}$          &  & 94.69${\pm 0.06}$          & 69.88${\pm 0.43}$          &  & 93.30${\pm 0.52}$          & 59.50${\pm 1.28}$          &  & 90.92${\pm 0.40}$          & 54.76${\pm 0.61}$          \\ \midrule
GCN                         &  & 89.31${\pm 0.43}$          & 81.59${\pm 0.61}$          &  & 89.56${\pm 3.66}$          & 78.10${\pm 0.43}$          &  & $82.56{\pm 1.92}$          & 70.35${\pm 0.41}$          &  & 90.47${\pm 0.24}$          & 81.50${\pm 0.53}$          \\
GAT                         &  & 90.85${\pm 0.23}$          & 82.75${\pm 0.36}$          &  & 91.46${\pm 1.82}$          & 78.21${\pm 0.44}$          &  & 86.48${\pm 1.50}$          & 71.58${\pm 0.80}$          &  & 93.17${\pm 0.20}$          & 83.03${\pm 0.50}$          \\
GraphSAGE                   &  & 90.41${\pm 0.53}$          & 82.19${\pm 0.45}$          &  & 86.21${\pm 0.82}$          & 77.45${\pm 2.38}$          &  & 92.05${\pm 0.39}$          & 67.51${\pm 0.76}$          &  & 85.51${\pm 0.50}$          & 77.90${\pm 2.50}$          \\
SGC                         &  & 89.83${\pm 0.32}$          & 80.59${\pm 0.16}$          &  & 94.10${\pm 0.12}$          & 78.84${\pm 0.18}$          &  & 91.35${\pm 1.68}$          & 71.44${\pm 0.75}$          &  & 91.50${\pm 0.21}$          & 81.32${\pm 0.50}$          \\ \midrule
HGNN                        &  & 96.42${\pm 0.44}$          & 84.71${\pm 0.98}$          &  & 92.75${\pm 0.26}$          & 77.13${\pm 0.82}$          &  & 93.58${\pm 0.33}$          & 69.99${\pm 1.00}$          &  & 91.67${\pm 0.41}$          & 78.26${\pm 1.19}$          \\
HGCN                        &  & 96.43${\pm 0.12}$          & 89.26${\pm 1.27}$          &  & 95.13${\pm 0.14}$          & 76.53${\pm 0.64}$          &  & 96.63${\pm 0.09}$          & 68.04${\pm 0.59}$          &  & 93.81${\pm 0.14}$          & 78.03${\pm 0.98}$          \\
HGAT                        &  & 97.86${\pm 0.09}$          & 89.62${\pm 1.03}$          &  & 94.18${\pm 0.18}$          & 77.42${\pm 0.66}$          &  & 95.84${\pm 0.37}$          & 68.64${\pm 0.30}$          &  & \textbf{94.02${\pm 0.18}$} & 78.32${\pm 1.39}$          \\
HyboNet                     &  & 97.30${\pm 0.30}$          & 90.90${\pm 1.40}$          &  & 95.80${\pm 0.20}$          & 78.00${\pm 1.00}$          &  & 96.70${\pm 0.80}$          & 69.80${\pm 0.60}$          &  & 93.60${\pm 0.30}$          & 80.20${\pm 1.30}$          \\ \midrule
\textcolor{blue}{HGDE}  &  & \textbf{98.9${\pm 0.20}$} & \textbf{95.10${\pm 0.30}$} &  & \textbf{96.20${\pm 0.20}$} & \textbf{81.5${\pm 0.30}$} &  & \textbf{96.70${\pm 0.70}$} & \textbf{74.10${\pm 0.50}$} &  & 94.00${\pm 0.70}$          & \textbf{84.20${\pm 0.60}$} \\ \bottomrule
\end{tabular}

==> table/lp_only.tex <==
\begin{tabular}{@{}lrrrrr@{}}
\toprule
Dataset     & Disease                     & Airport                     & PubMed                      & CiteSeer                    & Cora                      \\ \midrule
$\delta$    & $0$                         & $1$                         & $3.5$                       & $5$                         & $11$                      \\ \midrule
MLP         & 69.9$_{\pm   3.4}$          & 68.9$_{\pm   0.5}$          & 83.3$_{\pm   0.6}$          & 93.7$_{\pm   0.6}$          & 83.3$_{\pm   0.6}$        \\
HNN         & 70.2$_{\pm   0.1}$          & 80.6$_{\pm   0.5}$          & 94.7$_{\pm   0.1}$          & 93.3$_{\pm   0.5}$          & 90.9$_{\pm   0.4}$        \\ \midrule
GCN         & 64.7$_{\pm   0.5}$          & 89.3$_{\pm   0.4}$          & 89.6$_{\pm   3.7}$          & 82.6$_{\pm   1.9}$          & 90.5$_{\pm   0.2}$        \\
GAT         & 69.8$_{\pm   0.3}$          & 90.9$_{\pm   0.2}$          & 91.5$_{\pm   1.8}$          & 86.5$_{\pm   1.5}$          & 93.2$_{\pm   0.2}$        \\
SAGE        & 65.9$_{\pm   0.3}$          & 90.4$_{\pm   0.5}$          & 86.2$_{\pm   0.8}$          & 92.1$_{\pm   0.4}$          & 85.5$_{\pm   0.5}$        \\
SGC         & 65.1$_{\pm   0.2}$          & 89.8$_{\pm   0.3}$          & 94.1$_{\pm   0.1}$          & 91.4$_{\pm   1.7}$          & 91.5$_{\pm   0.2}$        \\ \midrule
HGCN        & 91.2$_{\pm   0.6}$          & 96.4$_{\pm   0.1}$          & 95.1$_{\pm   0.1}$          & 96.6$_{\pm   0.1}$          & 93.8$_{\pm   0.1}$        \\
$\kappa$GCN & 92.0$_{\pm   0.5}$          & 92.5$_{\pm   0.5}$          & 94.9$_{\pm   0.3}$          & 95.1$_{\pm   0.6}$          & 92.6$_{\pm   0.4}$        \\
LGCN        & 96.6$_{\pm   0.6}$          & 96.0$_{\pm   0.6}$          & 96.6$_{\pm   0.1}$          & 95.8$_{\pm   0.4}$          & 93.6$_{\pm   0.4}$        \\
HyboNet     & \textbf{96.8$_{\pm   0.4}$} & 97.3$_{\pm   0.3}$          & 95.8$_{\pm   0.2}$          & \textbf{96.7$_{\pm   0.8}$} & 93.6$_{\pm   0.3}$        \\ \midrule
HGDE-m        & 96.6$_{\pm   0.5}$          & \textbf{98.2$_{\pm   0.2}$} & \textbf{96.6$_{\pm   0.2}$} & 96.1$_{\pm   0.7}$          & \textbf{95.2$_{\pm 0.1}$} \\ \bottomrule
\end{tabular}

==> table/nc_only.tex <==
\begin{tabular}{@{}lrrrrr@{}}
\toprule
\textbf{Dataset} & \textbf{Disease}            & \textbf{Airport}            & \textbf{PubMed}             & \textbf{CiteSeer}           & \textbf{Cora}             \\ \midrule
$\delta$         & $0$                         & $1$                         & $3.5$                       & $5$                         & $11$                      \\ \midrule
MLP              & 32.5$_{\pm   1.1}$          & 60.9$_{\pm   3.4}$          & 72.4$_{\pm   0.2}$          & 59.5$_{\pm   0.9}$          & 51.6$_{\pm   1.3}$        \\
HNN              & 45.5$_{\pm   3.3}$          & 80.6$_{\pm   0.5}$          & 69.9$_{\pm   0.4}$          & 59.5$_{\pm   1.2}$          & 54.7$_{\pm   0.6}$        \\ \midrule
GCN              & 69.7$_{\pm   0.4}$          & 81.6$_{\pm   0.6}$          & 78.1$_{\pm   0.4}$          & 70.3$_{\pm   0.4}$          & 81.5$_{\pm   0.5}$        \\
GAT              & 70.4$_{\pm   0.4}$          & 82.7$_{\pm   0.4}$          & 78.2$_{\pm   0.4}$          & 71.6$_{\pm   0.8}$          & 83.0$_{\pm   0.5}$        \\
SAGE             & 69.1$_{\pm   0.6}$          & 82.2$_{\pm   0.5}$          & 77.5$_{\pm   2.4}$          & 67.5$_{\pm   0.7}$          & 79.9$_{\pm   2.5}$        \\
SGC              & 69.5$_{\pm   0.2}$          & 80.6$_{\pm   0.2}$          & 78.8$_{\pm   0.2}$          & 71.4$_{\pm   0.8}$          & 81.3$_{\pm   0.5}$        \\ \midrule
HGCN             & 82.8$_{\pm   0.8}$          & 89.2$_{\pm   1.3}$          & 80.3$_{\pm   0.3}$          & 68.0$_{\pm   0.6}$          & 79.9$_{\pm   0.2}$        \\
$\kappa$GCN      & 82.1$_{\pm   1.1}$          & 84.4$_{\pm   0.4}$          & 78.3$_{\pm   0.6}$          & 71.1$_{\pm   0.6}$          & 80.8$_{\pm   0.6}$        \\
LGCN             & 84.4$_{\pm   0.8}$          & 90.9$_{\pm   1.0}$          & 78.8$_{\pm   0.5}$          & 71.1$_{\pm   0.3}$          & 83.3$_{\pm   0.5}$        \\
HyboNet          & \textbf{96.0$_{\pm   1.0}$} & 90.9$_{\pm   1.4}$          & 78.0$_{\pm   1.0}$          & 69.8$_{\pm   0.6}$          & 80.2$_{\pm   1.3}$        \\ \midrule
HGDE-s             & 92.1$_{\pm   1.6}$          & \textbf{94.7$_{\pm   0.4}$} & \textbf{81.5$_{\pm   0.3}$} & \textbf{73.8$_{\pm   0.5}$} & \textbf{84.2$_{\pm 0.6}$} \\ \bottomrule
\end{tabular}

==> table/result_various_depth_backup.tex <==
\begin{tabular}{@{}clccccc@{}}
\toprule
\multirow{2}{*}{\textbf{}}                                                      & \multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c}{\textbf{Layers}}                                                                                                        \\ \cmidrule(l){3-7} 
                                                                                &                                 & 2                         & 8                         & 16                        & 32                         & 64                        \\ \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Airport}}}  & GCN                             & 78.1$_{\pm 1.5}$ & \textbf{83.2$_{\pm 4.7}$}          & 47.0$_{\pm 1.4}$          & 47.0$_{\pm 1.4}$           & 47.0$_{\pm 1.4}$          \\
                                                           & GCNII                           & 86.9$_{\pm 2.1}$          & 88.3$_{\pm 2.1}$          & \textbf{88.3$_{\pm 1.2}$} & 86.6$_{\pm 1.2}$           & 86.6$_{\pm 2.3}$          \\
                                                           & HGCN                            & \textbf{89.3$_{\pm 1.2}$} & 86.9$_{\pm 4.3}$          & 52.8$_{\pm 8.6}$          & 47.2$_{\pm 1.2}$           & 44.5$_{\pm 1.6}$          \\
                                                           & DeepHGCN                        & 89.7$_{\pm 1.9}$          & \textcolor{red}{\textbf{94.7$_{\pm 0.9}$}} & 92.9$_{\pm 1.2}$         & 93.1$_{\pm 0.9}$           & 92.5$_{\pm 1.3}$          \\ \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{PubMed}}}   & GCN                             & \textbf{78.1$_{\pm 0.5}$} & 40.7$_{\pm 0.0}$          & 40.7$_{\pm 0.0}$          & 40.7$_{\pm 0.0}$           & 40.7$_{\pm 0.0}$          \\
                                                           & GCNII                           & 77.9$_{\pm 0.8}$          & 76.9$_{\pm 2.5}$          & 78.5$_{\pm 1.0}$          & \textcolor{red}{\textbf{79.4$_{\pm 0.5}$}}  & 79.1$_{\pm 0.8}$          \\
                                                           & HGCN                            & \textbf{76.5$_{\pm 0.6}$} & 56.0$_{\pm 5.2}$          & 54.2$_{\pm 7.5}$          & 45.3$_{\pm 6.9}$           & 43.7$_{\pm 1.5}$          \\
                                                           & DeepHGCN                        & 78.0$_{\pm 0.4}$          & 78.1$_{\pm 0.7}$          & 78.5$_{\pm 0.5}$          & \textbf{79.4$_{\pm 0.9}$}  & 79.0$_{\pm 0.6}$          \\ \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{CiteSeer}}} & GCN                             & \textbf{71.0$_{\pm 1.0}$} & 18.1$_{\pm 0.0}$          & 18.1$_{\pm 0.0}$          & 18.1$_{\pm 0.0}$           & 18.1$_{\pm 0.0}$          \\
                                                           & GCNII                           & 54.7$_{\pm 7.4}$          & 56.1$_{\pm 6.1}$         & 66.5$_{\pm 6.2}$         & \textbf{69.4$_{\pm 1.8}$} & 68.6$_{\pm 1.8}$         \\
                                                           & HGCN                            & \textbf{68.0$_{\pm 0.6}$} & 39.5$_{\pm 7.1}$          & 30.3$_{\pm 3.7}$          & 31.2$_{\pm 4.9}$           & 24.7$_{\pm 1.3}$          \\
                                                           & DeepHGCN                        & 72.7$_{\pm 0.5}$          & 70.8$_{\pm 0.8}$          & 71.9$_{\pm 0.8}$          & 72.7$_{\pm 0.5}$           & \textcolor{red}{\textbf{73.3$_{\pm 0.4}$}} \\ \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Cora}}}     & GCN                             & \textbf{81.9$_{\pm 1.1}$} & 31.9$_{\pm 0.0}$          & 31.9$_{\pm 0.0}$          & 31.9$_{\pm 0.0}$           & 31.9$_{\pm 0.0}$          \\
                                                           & GCNII                           & 78.0$_{\pm 3.0}$          & 76.4$_{\pm 2.2}$          & 77.2$_{\pm 3.5}$          & 83.7$_{\pm 0.9}$           & \textcolor{red}{\textbf{84.0$_{\pm 1.3}$}} \\
                                                           & HGCN                            & \textbf{78.1$_{\pm 0.9}$} & 33.5$_{\pm 5.5}$          & 30.8$_{\pm 3.9}$          & 24.1$_{\pm 7.3}$           & 21.7$_{\pm 7.8}$          \\
                                                           & DeepHGCN                        & 82.5$_{\pm 0.5}$          & \textbf{83.6$_{\pm 0.4}$}         & 82.7$_{\pm 1.0}$          & 82.4$_{\pm 0.6}$           & 83.1$_{\pm 0.7}$ \\ \bottomrule
\end{tabular}

